Robot Learning on the Job: Human-in-the-Loop Autonomy and Learning During Deployment

With the rapid growth of computing powers and recent advances in deep learning, we have witnessed impressive demonstrations of novel robot capabilities in research settings. Nonetheless, these learning systems exhibit brittle generalization and require excessive training data for practical tasks. To harness the capabilities of state-of-the-art robot learning models while embracing their imperfections, we present Sirius, a principled framework for humans and robots to collaborate through a division of work. In this framework, partially autonomous robots are tasked with handling a major portion of decision-making where they work reliably; meanwhile, human operators monitor the process and intervene in challenging situations. Such a human-robot team ensures safe deployments in complex tasks. Further, we introduce a new learning algorithm to improve the policy's performance on the data collected from the task executions. The core idea is re-weighing training samples with approximated human trust and optimizing the policies with weighted behavioral cloning. We evaluate Sirius in simulation and on real hardware, showing that Sirius consistently outperforms baselines over a collection of contact-rich manipulation tasks, achieving an 8% boost in simulation and 27% on real hardware than the state-of-the-art methods in policy success rate, with twice faster convergence and 85% memory size reduction. Videos and more details are available at https://ut-austin-rpl.github.io/sirius/

==> main/4_approach_old.tex <==
\section{Method} 
\label{sec:method}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/model_final_corrected.pdf}
    \caption{\textbf{Overview of our human-in-the-loop learning model.}
    We maintain an ever-growing database of diverse experiences spanning four categories: human demonstrations, autonomous robot data, human interventions, and transitions preceding interventions which we call pre-interventions.
    We employ weighted behavioral cloning to learn vision-based policies from these experiences.
    We set weights according to these four categories, with a high weight given to interventions over other categories.
    }
    % \vspace{-1mm}
    \label{fig:model}
\end{figure}

We develop a policy learning method that makes best use of the deployment data to update the models in consecutive rounds. Devising a suitable learning algorithm is challenging due to data distribution shifts. As we discussed in Section~\ref{sec:properties}, the dataset is multi-modal, of mixed quality, and ever-growing.
To utilize such data sources, we have a critical insight that human interventions provide informative signals of task structure and human trust, which we will use to guide the design of our algorithm.

The core idea of our approach is to use human interventions to re-weigh training samples based on an approximate quality score. With these weighted samples, we train the policy with the weighted behavioral cloning method to learn the policy on mixed-quality data.
Our intuition is that with a mixed-quality dataset, different weight assignments can differentiate high-quality samples from low-quality ones, such that the algorithm prioritizes high-quality samples for learning.
This strategy has been shown effective in recent literature on offline reinforcement learning~\cite{nair2021awac,wang2020critic, Kumar2020ConservativeQF}. 
% 
In the following, we will review the weighted behavioral cloning method and discuss our method for learning the sample weights from human interventions.



% \new{}In our case, we would like to learn a state-action value function $Q^H_\pi(s,a)$ based on the human feedback information during the human-robot partnership. Our weights in the weighted BC framework will be a function of it, $w(s,a) = f(Q^H_\pi(s,a))$.



\begin{algorithm}
\caption{Learning at Deployment}
\label{alg:learning-deploy}
\begin{algorithmic}
\State Initialize memory buffer $\mathcal{D}$ with fixed size $L$ 
\State
\State \code{warmstart phase}
\State Collect a few human demonstrations $\tau_{1}, \ldots, \tau_{M}$ 
\State Initialize BC policy $\pi_{\theta}$: 
\State \hspace*{2mm} $\theta^*=\arg \max _{\theta} \mathbb{E}_{(s, a) \sim \mathcal{D}}\left[\log \pi_{\theta}(a \mid s)\right]$
\vspace*{0.7mm}
\State $\mathcal{D} \leftarrow \mathcal{D} \cup\left\{\tau_{1}, \ldots, \tau_{M}\right\} $
\State
\State \code{deployment-learning loop}
\While {deployment continues} 
    \State \code{deployment}
    \State Collect rollout episodes $\tau_{1}, \ldots, \tau_{K} \sim p_{\pi_{\theta}}(\tau)$ 
    \State $\mathcal{D} \leftarrow \mathcal{D} \cup\left\{\tau_{1}, \ldots, \tau_{K}\right\} $
    \If{$|\mathcal{D}| > L$}
    \State reorganize $\mathcal{D}$ to the size $L$ 
    \EndIf
\State \code{learning}
\For{each gradient step}
\State Sample batch $\left(s, a, c\right) \sim \mathcal{D}$
\State $w(s,a,c) = P^*(c) / P(c)$ from Eq. \ref{eq:rebalanced-dist}
\State $\theta^*=\arg \max _{\theta} \mathbb{E}_{(s, a) \sim \mathcal{D}}\left[w(s,a,c) \cdot \log \pi_{\theta}(a \mid s)\right]$ 

\EndFor
\State Update $\pi_{\theta}$ for next round of deployment
\EndWhile
\end{algorithmic}
\end{algorithm}

\subsection{\new{Intervention-guided Weighting Scheme}}
\label{human-weighting-scheme}

\todo{Intuition and Motivation:}

We will now explain our general intuition of how to optimize the use of human information in the human-in-the-loop robot system. 

Our first intuition is that human intervention samples are highly important samples and should be prioritized in learning. 
Human operated samples are expensive to obtain and should be optimized in general;  
but human intervention occurs at task regions where the robot is unable to complete the task and requires help. These are the risk-sensitive task states, and therefore data at these regions are highly valuable. Therefore, these state-action pairs should be ranked high by the value function, and we should upweight the human intervention samples such that these samples will positively influence learning more.

Moreover, we should not only make use of \emph{what} human samples to use, but also \emph{when} the human samples take place. 
We make the critical observation that when the robot operates autonomously, it usually performs reasonable behaviors; but when it demands interventions, it is when the robot make mistakes or perform suboptimal behaviors.
Therefore, human interventions implicit signify human value judgement of the robot behavior: the samples before human interventions are less desirable and of lower quality. These samples should be downweighted to reduce their impact on learning.

\todo{One approach --- offline RL and specify rewards:}

We should make use of the human information to learn an appropriate value function of the state-action pairs in the samples so as to optimize learning. 
One potential approach would be to manually specify a human intervention reward, which penalizes samples before intervention and reward human intervention samples, learning a human intervention Q value function following works like \cite{wang2020critic, nair2021awac, Kostrikov2021OfflineRL}. 
However, effectively learning value estimates may be challenging if the dataset does not cover a sufficiently wide distribution of states and actions as shown in \cite{gulcehre2020rl, fu2020d4rl}. In the deployment setting, the data are all successful data under human supervision, making value learning hard as we shown later empirically in Section \ref{experiments}. Alternatively, we could directly use human intervention feedback to re-weigh training samples through a intervention-guided data rebalancing scheme.

\todo{Our approach:}

First, we adapt a simpler and more straightforward approach to identify and penalize the pre-intervention samples: We designate a segment of length $\ell$ before the start of each human intervention as another class \texttt{pre-intervention}. This is equivalent to first learning the Q value then thresholding it to make it binary \texttt{robot action} sample or \texttt{pre-intervention} sample. We find this approach to be a sample efficient way to save the need of learning an extra Q value function model; it is also equally generalizable as it reflects human preference and judgement pertaining to the specific interaction.

\todo{Interpretation of our method:}

In our intervention-guided weighting scheme, we use reweighting as a way to rebalance the distribution of the dataset. Recall that each sample $(s, a, r, c)$ in our dataset contains a data class type $c$ indicating whether the sample denotes a human demonstration action, robot action, or human intervention action; we also relabel some of the samples as pre-intervention, which are the samples before human intervention. Initially, the categories follow the initial distribution in the dataset: the human intervention constitutes a small percentage of the entire samples. We will now change the dataset distribution by adding a weight to the loss term of each sample. This increases the ratio of human intervention at the expense of the ratio of the robot action. On the other hand, we decrease the ratio of pre-intervention too. Note that the ratio of the demonstration remains unchanged as they are still important and useful samples to learn from.

Suppose the dataset $\mathcal{D}$ has total number of samples $N$, and $n_c$ is the number of samples that is class $c$, where $c \in$ \{$\texttt{demo}$, $\texttt{intv}$, $\texttt{preintv}$, and $\texttt{robot}$\}; we use $\mathcal{D}_c$ to represent the collection of samples in $\mathcal{D}$ that is of class $c$. The original data distribution is $P(c) = n_c / N$ for class $c$. The default BC objective under the original data distribution is:

\begin{equation} \label{eq:original-dist}
\begin{split}
& \hspace{5mm} \underset{\theta}{\arg \max} \  \underset{(s, a) \sim \mathcal{D}}{\mathbb{E}}\left[\log \pi_{\theta}(a \mid s)\right] \\ 
%& = \underset{\theta}{\arg \max} \frac{1}{N} \sum_i^N \left[\log \pi_{\theta}(a_i \mid s_i)\right] \\
%& = \underset{\theta}{\arg \max} \frac{1}{N} \sum_{c} \sum_i^{n_c} \left[\log \pi_{\theta}(a_i \mid s_i)\right] \\
%& = \underset{\theta}{\arg \max} \sum_{c} \frac{n_c}{N} \left[ \frac{1}{n_c} \sum_i^{n_c} \left[\log \pi_{\theta}(a_i \mid s_i)\right] \right] \\
& = \underset{\theta}{\arg \max} \ \underset{P(c)}{\mathbb{E}} \  \underset{(s, a) \sim \mathcal{D}_c}{\mathbb{E}} \left[\log \pi_{\theta}(a \mid s)\right]. 
\end{split}
\end{equation}

We would aim for a new data distribution after rebalancing, $P^*(c)$ for class $c$. In general, we want to boost up $P(\texttt{intv})$ such that $P^*(\texttt{intv}) > P(\texttt{intv})$, and bring down $P(\texttt{preintv})$ such that $P^*(\texttt{preintv}) < P(\texttt{preintv})$; $\sum_c P^*(c) = \sum_c P(c) = 1$. Since $P^*(\texttt{intv})$ now occupies a large proportion, the proportion of the normal samples will be squashed for these more useful samples accordingly. The weight $w(s,a)$ for the samples in each individual class $c$ is set according to $P^*(c)$, with $w(s,a) = P^*(c) / P(c)$:

\begin{equation} \label{eq:rebalanced-dist}
\begin{split}
& \hspace{5mm} \underset{\theta}{\arg \max} \ \underset{P(c)}{\mathbb{E}} \  \underset{(s, a) \sim \mathcal{D}_c}{\mathbb{E}} \left[ w(s,a) \log \pi_{\theta}(a \mid s)\right] \\
& = \underset{\theta}{\arg \max} \ \underset{P(c)}{\mathbb{E}} \  \underset{(s, a) \sim \mathcal{D}_c}{\mathbb{E}} \left[ \frac{P^*(c)}{P(c)} \log \pi_{\theta}(a \mid s)\right] \\
%& = \underset{\theta}{\arg \max} \ \underset{P(c)}{\mathbb{E}} \ \frac{P^*(c)}{P(c)} \  \underset{(s, a) \sim \mathcal{D}_c}{\mathbb{E}} \left[ \log \pi_{\theta}(a \mid s)\right] \\
& = \underset{\theta}{\arg \max} \ \underset{P^*(c)}{\mathbb{E}} \  \underset{(s, a) \sim \mathcal{D}_c}{\mathbb{E}} \left[\log \pi_{\theta}(a \mid s)\right]. \\
\end{split}
\end{equation} 

% \begin{aligned}
% & \hspace{5mm} \underset{\theta}{\arg \max} \  \underset{(s, a) \sim \mathcal{D}}{\mathbb{E}}\left[ w(s,a) \log \pi_{\theta}(a \mid s)\right] \\ 
% & = \underset{\theta}{\arg \max} \ \frac{1}{W} \  \underset{(s, a) \sim \mathcal{D}}{\mathbb{E}}\left[ w(s,a) \log \pi_{\theta}(a \mid s)\right] \\https://www.overleaf.com/project/63c62762e444df2664d6521b
% & = \underset{\theta}{\arg \max} \  \underset{(s, a) \sim \mathcal{D}}{\mathbb{E}}\left[ \frac{w(s,a)}{W} \ \log \pi_{\theta}(a \mid s)\right] \\
% & = \underset{\theta}{\arg \max} \ \mathbb{E}_{(s, a) \sim \mathcal{D^*}}\left[\log \pi_{\theta}(a \mid s)\right]
% \end{aligned}
% $$


% Rather than relying on advantage-based weights, we explicitly leverage the human intervention signals in the dataset to construct our weighting scheme.
% (see Figure~\ref{fig:model} for an overview).
% Recall that each sample $(s, a, r, c)$ in our dataset contains a data class type $c$ indicating whether the sample denotes a human demonstration action, robot action, or human intervention action.
% We assign the weight for each sample according to $c$, that is
% \begin{equation}
%   w(s, a, c) \propto W_c / N_c
%  \end{equation}
% where $N_c$ refers to the total number of samples in the dataset corresponding to data class $c$; and $W_c$ is a hyperparameter that represents the contribution of class type $c$ to the weighted BC objective.
% By dividing the weight over the number of class samples $N_c$, we ensure that the overall contribution of each class type to the weighted BC objective is $W_c$, regardless of the makeup of the dataset.
% This is an important feature of our method, allowing us to operate over varying datasets with the same set of fixed hyperparameters.

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/results_plot.pdf}
    \caption{\textbf{Quantitative evaluations.} We compare our method with human-in-the-loop learning, imitation learning, and offline reinforcement learning baselines. Our results in simulated and real-world tasks show steady performance improvements of the autonomous policies over rounds. Our model reports the highest performances in all four tasks after three rounds of deployments and policy updates. Solid line: human-in-the-loop; dashed line: offline learning on data from our method.}
    % \vspace{3mm}
    \label{fig:results}
\end{figure*}

% The weighting scheme described so far resembles similar weighting schemes proposed by prior work~\cite{mandlekar2020humanintheloop}.
% While promising, this weighting scheme has a critical limitation --- it treats all of the robot samples with the same weight $W_{\texttt{robot}}$ regardless of their quality.
% While the robot often performs reasonable behaviors, it can make mistakes that subsequently demand interventions.
% In practice, humans exhibit a response delay in performing corrective interventions, as they must first detect mistakes and react accordingly. 
% During this delay period, the robot's actions can be highly undesirable, which can hurt subsequent policy training. Therefore, we should down-weight the influence of these samples.
% To address this limitation, we introduce a simple heuristic of relabeling robot samples within $\ell$ timesteps preceding a window of intervention as a new \textit{pre-intervention} class $c = \texttt{preintv}$.
% We use a low weight to reduce the contribution of these samples.

\subsection{Memory Management}
\label{sec:memory-management}
As the deployment continues and the dataset increases, large data slows down training convergence and takes up excessive memory space. We hypothesize that forgetting (routinely discarding samples from memory) helps prioritize important and useful experiences for learning, speeding up convergence and even further improving policy.
Therefore, we examine strategies for managing the memory buffer. 

We assume that we have a fixed-size memory buffer.
Once we buffer becomes full, we replace existing samples with new samples.
% Since we know that human data is useful, we always retain \texttt{demo} and \texttt{intv} samples and we instead reject robot execution samples corresponding to the \texttt{robot} class. 
\new{}We would like to investigate the following question: With limited data storage and a never-ending deployment data flow, how do we absorb the most useful data and preserve more valuable information for learning? 

\new{}We consider five strategies for managing the memory buffer of deployment data. Each strategy tests out a different hypothesis listed below: 
\begin{enumerate}
    \item \textbf{LFI} (Least-Frequently-Intervened): first reject samples from trajectories with the least interventions. \\
    \emph{(Preserving the most human intervened trajectories keeps the most valuable human and critical state examples, which helps learning the most.)}
    \item \textbf{MFI} (Most-Frequently-Intervened): first reject samples from trajectories with the most interventions. \\
    \emph{(All successful robot trajectories are of higher quality than those trajectories that are intervened therefore betterr data for learning.)}
    \item \textbf{FIFO} (First-In-First-Out): reject samples in the order that they were added to the buffer. \\
    \emph{(Later data with a higher performing policy are higher quality data for learning.)}
    \item \textbf{FILO} (First-In-Last-Out): reject the most recently added samples first. \\
    \emph{(Initial data with a worse performing policy have greater state coverage and data diversity for learning.)}
    \item \textbf{Uniform}: reject samples uniformly at random. \\
    \emph{(Maximizing diversity of data sources works the best.)}
\end{enumerate}

% Each strategy operates on a different of assumptions and offers unique advantages.
% For example, in MFI the advantage of retaining trajectories with fewer interventions is that they contain high-quality samples, whereas, with LFI, trajectories with the most interventions reveal rare corner cases that retain the diversity of the dataset. 

\subsection{\new{}Implementation Details}
\label{imple_details}

% For the sample weights, we find that good weighting schemes favor weights that are higher for the intervention class, lower for the robot class, and near-zero for the pre-intervention class.
% Intuitively, human interventions serve as a crucial supervisory signal that guides the agent to recover from suboptimal behaviors, while pre-interventions denote suboptimal behaviors.
% We set the weights as follows: $W_{\texttt{demo}} = N_{\texttt{demo}}/N$, $W_{\texttt{intv}} = 0.5$,  and $W_{\texttt{preintv}} = 0.002$, $W_{\texttt{robot}} = 1 - W_{\texttt{intv}} - W_{\texttt{demo}} - W_{\texttt{preintv}}$,
% where $N$ denotes the total number of samples in the memory.

In practice, we set $P^*(\texttt{intv}) = \frac{1}{2}$. The \texttt{demo} weight maintains the true ratio of demonstration samples in the dataset: $P^*(\texttt{demo}) = P(\texttt{demo}) = n_\texttt{demo} / N$. Finally, $P^*(\texttt{robot})$ adjusts itself accordingly: $P^*(\texttt{robot}) = 1 - P^*(\texttt{demo}) - P^*(\texttt{robot})$. Note how the demonstrations have their original ratio preserved --- it keeps the policy close to the expert data distribution, especially during initial rounds of updates when the robot generates lower-quality data. This is in contrast to Mandlekar et al.~\cite{mandlekar2020humanintheloop} which treats all non-intervention samples as a single class, thus lowering the contribution of demonstrations over time. The actual weight for each sample $w(s,a,c) = P^*(c) / P(c)$, as discussed in Section \ref{human-weighting-scheme}.

In practice, since we are in a long-term deployment setting where most data are robot actions, and interventions only happen at critical regions in a trajectory, we can safely assume that $P(\texttt{intv}) < \frac{1}{2}$. For the same reason, the few demonstrations which we use to bootstrap the learning loop are a small proportion of all deployment data, so $P^*(\texttt{demo}) = P(\texttt{demo}) < \frac{1}{2}$, such that $P^*(\texttt{robot}) = 1 - P^*(\texttt{demo}) - P^*(\texttt{robot}) - P^*(\texttt{preintv}) > 0$. We show that $P^*(\texttt{intv}) = \frac{1}{2}$ is a reasonable choice of hyperparamters in Section \ref{experiments} where we do an extensive study of how the specific weighting ratio hyperparameters affect learning. 


The optimal choice on the hyperparameter $\ell$ depends on \emph{Human Reaction Time}, which quantifies how fast the human operator reacted to the robot’s suboptimal behavior. Prior works \cite{hri_response_2022, spencer2020wil} indicate that a response delay exists between the time the robot starts to perform mistakes and the time human actually perform corrective interventions. Our empirical observation based on our human operator shows an average \emph{Human Reaction Time} of $2$ seconds. Our controller frequency is $20$ mHz and we put a $0.08$s time delay between each controller timestep for better human reaction to the robot, for a total of $0.05$s + $0.08$s = $0.13$s timestep interval. This roughly corresponds to $15$ timesteps of robot state-action pairs, which we will use to set $\ell$.

For the robot policy, we adopt BC-RNN~\cite{robomimic2021}, the state-of-the-art behavioral cloning algorithm, as our model backbone.
We use ResNet-18 encoders \cite{DBLP:journals/corr/HeZRS15} to encode third person and eye-in-hand images \cite{robomimic2021, mandlekar2020gti}.
We concatenate image features with robot proprioceptive state as input to the policy.
The network outputs a Gaussian Mixture Model (GMM) distribution over actions. See Appendix \ref{app:imple_tables} for the full details.




